Rate of Convergence of Attractors for Singularly Perturbed Semilinear Problems

We exhibit a class of singularly perturbed parabolic problems which the asymptotic behavior can be described by a system of ordinary differential equation. We estimate the convergence of attractors in the Hausdorff metric by rate of convergence of resolvent operators. Application to spatial homogenization and large diffusion except in a neighborhood of a point will be considered.

==> References.tex <==
% This file was created with JabRef 2.10b2.
% Encoding: UTF-8


@Book{A.N.Carvalho2010a,
  Title                    = {Attractors for infinite-dimensional non-autonomous dynamical systems},
  Author                   = {A. N. Carvalho, J.A. Langa, J.C. Robinson,},
  Editor                   = {Springer},
  Year                     = {2010},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{flank,
  Title                    = {Rate of convergence of Attractors for some sinsingular perturbed parabolic problems},
  Author                   = {J. M. Arrieta and F.D.M. Bezerra and A. N. Carvalho},
  Journal                  = {Top. Methdos Nonlinear Anal},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{J.M.Arrieta2000,
  Title                    = {Attractors for parabolic pro\-blems with nonlinear boundary bondition. Uniform bounds},
  Author                   = {J. M. Arrieta and A. N. Carvalho and A. Rodr{\'\i}guez-Bernal},
  Journal                  = {Commun. in partial differential equations},
  Year                     = {2000},
  Pages                    = {1-37},
  Volume                   = {25},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{J.M.Arrieta2000a,
  Title                    = {Upper semicontinuity for attractors of parabolic problems with localized large diffusion and nonlinear boundary conditions},
  Author                   = {J. M. Arrieta and A. N. Carvalho and A. Rodr{\'\i}guez-Bernal},
  Journal                  = {Journal of Differential Equations},
  Year                     = {2000},
  Pages                    = {33-59},
  Volume                   = {168},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{J.M.Arrieta1999,
  Title                    = {Parabolic problems with nonlinear boundary conditions and critical nonlinearities},
  Author                   = {J. M. Arrieta and A. N. Carvalho and A. Rodr{\'\i}guez-Bernal},
  Journal                  = {Journal of Differential Equations},
  Year                     = {1999},
  Pages                    = {376-406},
  Volume                   = {156},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{Carbone2006,
  Title                    = {Continuity of the attractors in a singular problem arising in composite materials},
  Author                   = {V. L. Carbone and J. G. Ruas-Filho},
  Journal                  = {Nonlinear Anal},
  Year                     = {2006},
  Pages                    = {1285-1305},
  Volume                   = {65},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{Carvalho2010,
  Title                    = {Equi-exponential attraction and rate of convergence of attractors for singularly pertubed evolution equations},
  Author                   = {A.N. Carvalho and J.W. Cholewa and T.Dlotko},
  Journal                  = {Cadernos de matemática},
  Year                     = {2010},
  Pages                    = {111-151},
  Volume                   = {11},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{E.R.Aragao-Costa2011,
  Title                    = {Stability of gradient semigroups under perturbations},
  Author                   = {E.R. Aragão-Costa, T. Caraballo, A. N. Carvalho, J.A.Langa},
  Journal                  = {Nonlinearity},
  Year                     = {2011},
  Volume                   = {24},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Book{Henry1980a,
  Title                    = {Geometric theory of semilinear parabolic equations},
  Author                   = {Dan Henry},
  Editor                   = {Springer-Verlag},
  Publisher                = {Lecture Notes in Mathe\-matics},
  Year                     = {1980},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@PhdThesis{Pires2013,
  Title                    = {Taxa de atração para equações com difusão grande localizada},
  Author                   = {Leonardo Pires},
  School                   = {UfSCar},
  Year                     = {2013},
  Type                     = {Dissetação de mestrado},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{Santamaria2014,
  Title                    = {Estimates on the distance of inertial manifolds},
  Author                   = {E. Santamaria and J. M. Arrieta},
  Journal                  = {Discrete and continuous dinamical systems},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {3921-3944},
  Volume                   = {34},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}


